From Summary to Action: Enhancing Large Language Models for Complex Tasks with Open World APIs

The distinction between humans and animals lies in the unique ability of humans to use and create tools. Tools empower humans to overcome physiological limitations, fostering the creation of magnificent civilizations. Similarly, enabling foundational models like Large Language Models (LLMs) with the capacity to learn external tool usage may serve as a pivotal step toward realizing artificial general intelligence. Previous studies in this field have predominantly pursued two distinct approaches to augment the tool invocation capabilities of LLMs. The first approach emphasizes the construction of relevant datasets for model fine-tuning. The second approach, in contrast, aims to fully exploit the inherent reasoning abilities of LLMs through in-context learning strategies. In this work, we introduce a novel tool invocation pipeline designed to control massive real-world APIs. This pipeline mirrors the human task-solving process, addressing complicated real-life user queries. At each step, we guide LLMs to summarize the achieved results and determine the next course of action. We term this pipeline `from Summary to action', Sum2Act for short. Empirical evaluations of our Sum2Act pipeline on the ToolBench benchmark show significant performance improvements, outperforming established methods like ReAct and DFSDT. This highlights Sum2Act's effectiveness in enhancing LLMs for complex real-world tasks.

==> sec/3_method.tex <==
\section{Method}
Our model Sum2Act leverage a large language model and expansive open-world APIs to solve real-world tasks. 
Sum2Act first utilizes a retriever to obtain relevant tools(or APIs) based on the correlation between user instructions and descriptions or tools(or APIs).
Then it operates in three critical stages: task identification, action proposal, and summarization, as depicted in Figure~\ref{fig:pipeline}.
Upon receiving a user's instruction, the task planner initially identifies the target task and dissects it into several subtasks according to the tools. 
Then, Sum2Act goes through an iterative cycle between the task proposal stage and the summarization stage. 
In the task proposal stage, the router evaluates its progress, determining whether to conclude the task or propose a tool for further action. 
Subsequently, in the summarization stage, the state manager assesses the observations of these actions, updating the overall state accordingly.
%The process ends when the system either completes the task and offers a solution, or recognizes the task as unachievable and opts to discontinue its efforts.
The process ends when Sum2Act completes the task and offers a solution. We briefly depict our algorithm in  \cref{alg:Sum2Act}.

\begin{algorithm}[ht]
  \caption{Sum2Act}
  \label{alg:Sum2Act}
  \KwIn{User instruction: $I$.}
  \KwData{LLM: $\mathcal{M}$; API Retriever: $\mathcal{R}$; Initial state: $S_0$; Prompts: $\mathrm{prompt}$.}
  \KwOut{Answer: $Answer$.}
  \BlankLine
  Initialize state $S=S_0$\; 
  \tcp{0. Get relevant APIs}\
  $Tools=\mathcal{R}(I)$\\
  \tcp{1. Task identification Stage}
   $Task=\mathcal{M}\left(\mathrm{prompt}_{\mathrm{task}},I,Tools\right)$\; 
  \While{True}{
  \tcp{2. Action Proposal Stage}
 $Action,Args=\mathcal{M}\left(\mathrm{prompt}_{\mathrm{plan}},Task,S,Tools\right)$\;
  \If{$Action==``\mathrm{Finish}"$}{
    {\bf break}\;
  }
  $observation=Action(Args)$;\\
  \tcp{3. Summarization Stage}
  $S=\mathcal{M}\left(\mathrm{prompt}_{\mathrm{state}}, observation, Task, S\right)$;\\
  }
  $Answer = Args[``\mathrm{Answer}"]$\;
\end{algorithm}


\subsection{Task Identification}
User instructions often encompass problem descriptions and polite language, while the target task typically features relatively straightforward content. 
To proficiently handle this process, the task planner first identifies the user's target task from the given instruction. Simultaneously, it decomposes the identified task into several potential subtasks based on the relevant tools.
Specifically, We utilize a large language model, denoted as $\mathcal{M}$, with a specific prompt $\mathrm{prompt}_{\mathrm{task}}$, to facilitate this process during the task identification state. This can be expressed as:
\begin{equation}
Task = \mathcal{M}\left(\mathrm{prompt}_{task}, I,Tools\right)
\end{equation}
\begin{equation}
Task = \left\{TargetTask;{subtask}_1, \ldots, {subtask}_n\right\}
\end{equation}
Where $I$ is the user instruction, $Tools$ are the tools retrieved by the retriever, ${TargetTask}$ represents the target task, ${subtask}_i$ indicates the $i$-th subtask, and $n$ is the total number of subtasks.
Collectively, the target task and its subtasks are referred to as ${Task}$.

The task identification stage is distinct from the task planning stage. At this stage, the role of the task planner is solely to identify and break down the target task from the user instruction. It does not engage in tool selection or application strategies. 
This stage has two main objectives: (1) filter out extraneous information, focusing exclusively on identifying and decomposing the target task, and (2) ensure that the identified target task and its subtasks are more conducive to subsequent stages than the raw user instructions.
Following the task identification stage, Sum2Act iteratively navigates through the action proposal and summarization stages. 
This cycle continues until a termination condition is reached, signifying the completion of the process.

\subsection{Action Proposal}
At the action proposal stage, the router will plan the next action and then execute it. 
% To facilitate reasoning and planning for the router, 
To enhance the decision-making capabilities of the router, we utilize the task acquired in the task identification stage instead of relying on the raw user instruction. 
This approach better enables the router to assess what tasks are at hand and determine the next action to be taken.
Specifically, we employ a language model $\mathcal{M}$ and well designed prompt $\mathrm{prompt}_{\mathrm{plan}}$ to act as the router. 
The router engages in thought and reasoning based on the current state, the task, and available tools, subsequently choosing the next action and the arguments of the action.
This process can be formalized as follows:
\begin{equation}
{Action},{Args} = \mathcal{M}(\mathrm{prompt}_{\mathrm{plan}},{Task},{S},Tools)
\end{equation}
$Action$ can represent either one of the tools or the special action $``\mathrm{Finish}"$, signifying the completion of the target task.
\begin{itemize}
    \item If the value of $Action$ is not $``\mathrm{Finish}''$, it indicates that, from the router's perspective, the target task has not been completed. In this scenario, $Action$ denotes a specific tool or API, and $Args$ encapsulate the corresponding arguments for the given $Action$. The router proceeds to execute the specified action, subsequently obtaining relevant observations in the process.
    \begin{equation}
        observation = Action\left(Args\right)
    \end{equation}
    \item If the value of $Action$ is exactly $``\mathrm{Finish}''$, it indicates that the router perceives the target task as completed. In such a scenario, the program will exit the loop, provide a response to the user's command, and ultimately terminate. The variable $Args$ contains the answer utilized to respond to the user. 
    \begin{equation}
        Answer = Args[``\mathrm{Answer}"]
    \end{equation}
\end{itemize}

\subsection{Summarization}
% 多写写
% the most different point
Subsequent to the action proposal stage, Sum2Act transitions into a novel stage we have termed the "summarization" stage. 
At this stage, the central component is the state manager, which is responsible for maintaining the {\bf State} of the system.

% 讲 motivation
We draw inspiration from the human working process: when an individual is engaged in a complex task, they periodically summarize their progress, noting what has been completed and challenges encountered. The summarization process involves effectively processing the outcomes of past actions, highlighting significant results, filtering out task-irrelevant information, and aiding in subsequent planning for the individual.

Distinct from the conventional memory structure used in many reasoning methods, the {\bf State} in our system is a dynamic representation of the current scenario, informed by all observations of preceding actions.
This differs from traditional memory, which primarily logs observations from past actions without an evolving contextual understanding.

The {\bf State} comprises two primary elements:
\begin{itemize}
\item {\it Current results}: This aspect reflects the ongoing progress toward task completion.
\item {\it Failure history}: This records any issues encountered with tools, guiding the router to avoid repeat selections of problematic options.
\end{itemize}

% stress the advantage of our method
In the Chain of Thought (CoT) process, the length of memory can become cumbersome as observations accumulate. Practical applications often resort to truncation methods to manage this, but such approaches invariably lead to information loss. This presents a fundamental trade-off: balancing the completeness of memory with its manageability.

The excessively elongated memory can impede efficiency and decision-making ability of the router due to the overload of irrelevant data. 
On the other hand, overly truncated memory can leave the router under-informed, especially when dealing with complex tasks.

To address this, the state manager synthesizes the observation and updates the {\bf State} accordingly after each action executed by the router. The process is formalized as follows:
\begin{equation}
S = \mathcal{M}(\mathrm{prompt}_{\mathrm{state}}, {observation}, {Task}, S)
\end{equation}
Here, ${observation}$ denotes the outcome of the tool's execution, while $\mathrm{prompt}_{\mathrm{state}}$ is the associated prompt. 
Contrary to the memory, the length of textual content within a state is maintained within reasonable limits. It encapsulates a summary of all previous actions' observations, thus minimizing information loss. Consequently, the information density within the state is typically much higher than that in memory, a crucial feature in open-world scenarios where APIs often yield extensive but irrelevant data.

Upon summarizing the observations and updating the {\bf State}, the state manager efficiently streamlines the decision-making process for subsequent actions.



==> table/compare.tex <==
\begin{table*}
    % \small
    % \setlength{\abovecaptionskip}{0pt}%    
% \setlength{\belowcaptionskip}{10pt}%
    \centering
    \begin{tabular}{ccccc}
        \toprule
        \multirow{2}*{Model}& \multirow{2}*{Method}&\multicolumn{2}{c}{Similarity Measure}&\multirow{2}*{Average}\\
        \cmidrule(r){4-5}
        &&&Inception V3$\uparrow$& CLIP$\uparrow$\\
        \midrule

      \bottomrule
      \end{tabular}
       \caption{\textbf{caption}}
       \label{tab:compare}
\end{table*}

==> table/task_extraction.tex <==
\begin{table*}[htb]
    \centering
  \begin{tabular}{p{0.1\linewidth}|p{0.7\linewidth}}
  \toprule
  Field & Prompt Description \\
  \midrule
  Target task & First of all, you need to identify which target task the user want you to do, note that the user's input may describe a global task but only parts of the task need to be done by you. \\
  \midrule
  subtasks & Then you need to decompose the target task into one or more subtasks which can be solved by the available API functions. \\
  \midrule
  format & "Target task": brief description of AI assistant's target task(input output information should be contained), 
  "Decomposed tasks": " Your target task may involve following subtasks: 1.brief subtask description--possible APIs to use 2.brief subtask description--possible APIs to use ..." \\
  \bottomrule
\end{tabular}
    \caption{Task Extraction}
    \label{tab:task_extract}
\end{table*}

